Space-time multilevel quadrature methods and their application for cardiac electrophysiology

We present a novel approach which aims at high-performance uncertainty quantification for cardiac electrophysiology simulations. Employing the monodomain equation to model the transmembrane potential inside the cardiac cells, we evaluate the effect of spatially correlated perturbations of the heart fibers on the statistics of the resulting quantities of interest. Our methodology relies on a close integration of multilevel quadrature methods, parallel iterative solvers and space-time finite element discretizations, allowing for a fully parallelized framework in space, time and stochastics. Extensive numerical studies are presented to evaluate convergence rates and to compare the performance of classical Monte Carlo methods such as standard Monte Carlo (MC) and quasi-Monte Carlo (QMC), as well as multilevel strategies, i.e. multilevel Monte Carlo (MLMC) and multilevel quasi-Monte Carlo (MLQMC) on hierarchies of nested meshes. Finally, we employ a recently suggested variant of the multilevel approach for non-nested meshes to deal with a realistic heart geometry.

==> numerical-experiments.tex <==
%========================================
\section{Numerical experiments}\label{sct:numerix}
%========================================
\subsection{Setup}
%========================================
The numerical experiments have been conducted for three
test-case geometries: a cube, an idealized ventricle and
a heart geometry (atria excluded) that was acquired through real
patient CCT data. We will refer to the latter geometry with
the term ``realistic heart''. The simulations have been realized
using \texttt{SLOTH}, see \cite{quaglino2017sloth}, a UQ 
Python library developed at the Institute of Computational 
Science (ICS) in Lugano. For this work, we extended it to 
the monodomain equation (and in general to all types of 
$3+1$ dimensional PDEs) by employing \texttt{Utopia}, 
see \cite{Zulian2017d}, for the finite element formulation. 

\paragraph{Parameters for the monodomain equation.} 
Regarding the models \eqref{monodomain} and \eqref{ionic_term}, 
we will always rely on the following parameters:    
\begin{itemize}
    \item The values for the ionic channel model $I_\text{ion}(u)$ in \eqref{ionic_term}
    are set as $\alpha = 1.4\cdot10^{-3}$ mV$^{-2}$ms$^{-1}$, 
    $u_\text{rest}=0$ mV, $u_\text{th}=28$ mV, and $u_\text{peak} = 115$ mV. 
    \item We choose
    \[
    I_{\text{app}}({\bs x},t) = \left( u_\text{rest} + u_\text{peak} \exp{ \left( - \dfrac{ ( {\bs x} - {\bs x}_0 )^2 }{ \sigma^2 } \right)} \right) \chi_{[0,t_1)}(t),
    \]
    where $t_1 = \Delta t = 0.005$ ms is the function we rely on for the 
    applied stimulus. Parameters $\sigma$ and ${\bs x}_0$ represent 
    respectively the power and the location of the stimulus. They are 
    geometry dependent.
\end{itemize}

\paragraph{Parameters for Karhunen-Lo\`eve expansion.} 
For the numerical experiments,
we introduce a scaling factor $\theta\in\RR$ into the covariance kernel
$\Cov[{\bs V}]$ to be able to easily scale the applied perturbation size.
The stochastic dimension $M$ in the computed, parametric Karhunen-Lo\`eve expansion
\eqref{eq:KLlowrank}
arises from prescribing the truncation error $\epsilon = 10^{-2}$ in the
pivoted Cholesky decomposition. The other parameters used in 
the Karhunen-Lo\`eve expansion differ from one experiment to 
another and are listed below:
\begin{itemize}
\item \textbf{Cube.} 
We consider isotropic diffusion and a scaling factor $\theta=0.3$ on 
\(D=[-0.5,0.5]^3\). 
The covariance matrix is induced by the scalar covariance kernel  
$\Cov[{\bs V}]({\bs x},{\bs x}') = \theta^2 e^{\frac{-\|{\bs x}-{\bs x}'\|_2^2}{\sigma_{\text{KL}}}}$
with $\sigma_{\text{KL}} =0.25$. The low-rank 
Cholesky approximation of the covariance matrix yielded the stochastic 
dimension $M = 66$. The mean diffusion is set to
$\Ebb[{\bs V}]({\bs x}) = 3.325\cdot 10^{-3}$mm$^2$ ms$^{-1}$ for all ${\bs x} \in D$. 
\item \textbf{Idealized ventricle.}  We consider isotropic diffusion 
and the scaling factor $\theta=0.3$. The covariance kernel is given 
by $ \Cov[{\bs V}]({\bs x},{\bs x}') = \theta^2 e^{\frac{-\|{\bs x}-{\bs x}'\|_2^2}
{\sigma_{\text{KL}}}}$ with $\sigma_{\text{KL}} =0.5$. The stochastic 
dimension is given by $M = 87$. The mean diffusion is set to 
$\Ebb[{\bs V}]({\bs x}) = 3.325\cdot 10^{-3}$mm$^2$ ms$^{-1}$
for all ${\bs x} \in D$. The domain's bounding box is given by
\([0.80,2.8]\times[1.01,3.5]\times[0.60,2.6]\).
\item \textbf{Heart geometry.} We consider anisotropic diffusion
with a block-diagonal covariance matrix given by 
$\Cov_{i,j}[{\bs V}]({\bs x},{\bs x}') = \delta_{i,j} \theta^2 e^{\frac{-\|{\bs x}-{\bs x}'\|_2^2} {\sigma_{\text{KL}}}}$
for $1 \leq i,j \leq 3$, where $\delta_{i,j}$ is the 
Kronecker delta. We set $\sigma_{\text{KL}} =0.16$. The scaling 
factor is set to $\theta=0.3$. The stochastic dimension is $M=135$. 
Furthermore, the perpendicular diffusion in \eqref{eq:AdmV} is 
chosen as $g=1.625\cdot 10^{-3}$mm$^2$ ms$^{-1}$
while $\Ebb[{\bs V}]({\bs x})$ is specified later.
The domain's bounding box is given by
\([-0.41,0.66]\times[0.21,1.03]\times[0.56,1.61]\).
\end{itemize}

\paragraph{Reference solution and error metrics.} 
In all the convergence and work comparison graphs that 
follow, the referenced root mean square error
in the $H^q$ norm ($L^2=H^0$ and $H^1$ for 
respectively $q=0$ and $q=1$) for
$\operatorname{QoI}_l = \operatorname{QoI}_l^{\text{SL}}$
or $\operatorname{QoI}_l = \operatorname{QoI}_l^{\text{ML}}$
is given by 
\begin{equation}\label{eq:space-time-error}
%%======================================
%e_l = \mathbb{E}\big[  \| u_l(\cdot) 
%- \mathbb{E} [u_{\text{ref}}(\cdot)] \|^2_{L^2((0,T);H^q(D))} \big]
e_l = \Big(\mathbb{E}\Big[\big\|\operatorname{QoI}_l[u] - \operatorname{QoI}_{\text{ref}}[u]\big\|_{L^2((0,T);H^q(D))}^2\Big]\Big)^{1/2}
\end{equation}
in case of a space--time quantity of interest,
such as the transmembrane potential,
\begin{equation}\label{eq:point-error}
%======================================
%e_l = \mathbb{E}\big[  \| u_l({\bs x}_0,\cdot) 
%- \mathbb{E} [u_{\text{ref}}({\bs x}_0,\cdot)] \|^2_{H^q(0,T)} \big],
e_l = \Big(\mathbb{E}\Big[\big\|\operatorname{QoI}_l[u] - \operatorname{QoI}_{\text{ref}}[u]\big\|_{H^q(0,T)}^2\Big]\Big)^{1/2}
\end{equation}
in case of a time quantity of interest,
such as the action potential at a given location ${\bs x}_0$ in space,
and
\begin{equation}\label{eq:activation-time-error}
%======================================
e_l = \Big(\mathbb{E}\Big[\big|\operatorname{QoI}_l[u] - \operatorname{QoI}_{\text{ref}}[u]\big|^2\Big]\Big)^{1/2}
\end{equation}
in the case of a scalar quantity of interest,
such as the activation time at a given point ${\bs x}_0$ in space.
Note that the mean in the above expressions is taken over the realisations
of the possibly non-deterministic quadrature formulas.
Specifically, for the Monte Carlo quadrature, the expectation for 
both, the single-level and multilevel runs, are approximated 
by averaging over 10 simulations at each level of precision 
for the nested case study, and 5 simulations for the 
non--nested example.
The reference quantity of interest $\operatorname{QoI}_{\text{ref}}[u]$
is computed by using $N=\text{10'000}$ samples drawn from the Halton sequence. 

The intergrid transfer of a space--time quantity of interest
from a given coarse level $l$ to the fine level $L$, required 
to evaluate the error \eqref{eq:space-time-error}, is 
performed by means of the tensor product of the space and 
time interpolation matrices.
%The transferred mesh function 
%is hence obtained by the matrix--vector multiplication
%$v_L = I^L_{l}  v_l$, where $v_l$ is the given discrete 
%mesh function at level $l$.
Obviously, the intergrid transfer of a time quantity of interest
from a given coarse level $l$ to the fine level $L$, required 
to evaluate the error \eqref{eq:point-error}, is 
performed analogously by means of the time interpolation matrices.

\paragraph{Quadrature methods.} 
In our experiments, we will consider the Monte Carlo
(MC) and quasi-Monte Carlo (QMC) quadrature method and
their multilevel pendants MLMC and MLQMC. Let us recall that 
the error is of order $2^{-2l}$ in the $L^2$ norm ($2^{-l}$ in the $H^1$ norm) when using 
linear finite elements of mesh size $h_l = 2^{-l}$. Therefore, in view
of the convergence rates for MC and QMC, the number of samples 
to be executed by these methods on a level $l$ to get the
same order of error $2^{-2l}$ is respectively given by 
\begin{equation}\label{eq:SampleNumbers}
%========================================
N_{\text{MC},l} = 2^{4l}\quad\text{and}
\quad N_{\text{QMC},l} = 2^{2l}.
\end{equation}
Regarding the $H^1$--error, the number of samples 
to be executed on a level $l$ to get the
same order of error $2^{-l}$ is respectively given by
\begin{equation}\label{eq:SampleNumbersH1}
%========================================
N_{\text{MC},l} = 2^{2l}\quad\text{and}
\quad N_{\text{QMC},l} = 2^{l}.
\end{equation}

%===============================================
\subsection{Scalar random diffusion for simple geometries and nested meshes}
%===============================================
In these first experiments, we consider a scalar, thus isotropic, 
random diffusion for the sake of simplicity. The experiments 
are conducted on the cube and the idealized ventricle geometry.
Note that the intergrid mesh transfer in case of the space--time 
dependent quantity of interest is straightforward as the meshes 
are nested.

%===============================================
\subsubsection{Cube geometry} 
%===============================================
We use a hierarchy of $L=6$ nested mesh 
levels. Starting from the finest level $l=L-1$, the coarser levels 
$l=0,1,\dots,L-2$ are successively obtained from the prior finer 
levels $l+1=1,2,\dots,L-1$ by uniformly coarsening in space and time.
The number of space-time degrees of freedom (DOF), the space 
and time discretization steps of all the different levels are 
reported in Table \ref{table:cube-levels}.

\begin{table}[h!]
\centering
\begin{tabular}{|c||l|l|l|l|l|l|} 
\hline $l$ & 0 &  1 & 2 & 3 & 4 & 5  \\
\hline
\hline DOF  & 16 & 256 & 4'096 & 65'536 & 1'048'576 & 16'777'216   \\
\hline
\hline $ h $  & 0.5 & 0.25 & 0.125 & 0.0625 & 0.03125 & 0.015625   \\
\hline $ \Delta t $  & 0.16 & 0.08 & 0.04 & 0.02 & 0.01 & 0.005   \\
\hline 
\end{tabular}
\caption{Details about the considered mesh hierarchy for the cube geometry.}
\label{table:cube-levels}
\end{table}

%========================================
\paragraph{Controlled convergence of the over-all error.}
%========================================
We intend to estimate and verify the convergence rate for 
the quadrature methods under consideration. The number of 
samples on each level is determined by the sampling strategy 
for controlling the error, cf.\ Section \ref{section:methods},
by using the sample numbers \eqref{eq:SampleNumbers} 
and \eqref{eq:SampleNumbersH1}. We  report in Figure 
\ref{fig::controlled-convergence-cube} the convergence of 
the error in $L^2$ and $H^1$ norms. 

The plots show that we recover the expected convergence 
rates of the general error for all quadrature methods tested. Note that this
does not imply that these quadrature methods are all equally efficient,
but rather that they yield the same precision with a vastly different balancing 
of samples on every level. This is demonstrated quite clearly in the corresponding
work comparison plot found in Figure \ref{fig::asymptotical-work-cube}.

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/eps/QMC_MC_MLMC_MLQMC_Contolled_Convegence_cube_L2_6levels.eps}
\includegraphics[width=0.45\textwidth]{figures/eps/QMC_MC_MLMC_MLQMC_Contolled_Convegence_cube_H1_6levels.eps}
\caption{Convergence rate for the cube in $L^2$ (left) and $H^1$ (right) norms.}
\label{fig::controlled-convergence-cube}
\end{figure} 


%========================================
\paragraph{Asymptotical work behaviour.}
%========================================
Equivalently to the controlled convergence concept with the previously 
introduced sampling strategy, we would like now to study the work in 
the context of the controlled error. To this end, we assume that the
cost per solve on level $l$ is given by $C_{\text{FE},l} = 2^{\gamma d l}$, 
where $\gamma$ is the complexity of the finite element solver used 
and $d$ is the dimension of the physical problem considered (here $d=4$). 
In view of \eqref{eq:SampleNumbers}, we can hence recover the 
total amount of work required by MC and QMC given a 
discretization level $L$ with \eqref{eq:SL} by
\[
W_{\text{MC},L} = C_{\text{FE},L} N_{\text{MC},L}
= 2^{\gamma d L} 2^{4L} = 2^{ (\gamma d + 4) L }
\]
and 
\[
W_{\text{QMC},L} = C_{\text{FE},L} N_{\text{QMC},L}
= 2^{\gamma d L} 2^{2L} = 2^{ (\gamma d + 2) L } . 
\]

The total work for the multilevel pendants with 
$L$ discretization levels can also be deduced from 
\eqref{eq:SampleNumbers} with \eqref{eq:StandardML}, and we can write 
\[
    W_{\text{MLMC},L} = \sum_{l=1}^{L} C_{\text{FE},L} N_{\text{MC},L-l} 
    = \sum_{l=1}^{L} 2^{\gamma d l} 2^{4(L-l)} =  2^{4L} \sum_{l=1}^{L} 2^{ (\gamma d - 4) l}
\]
and 
\[
    W_{\text{MLQMC},L} = \sum_{l=1}^{L} C_{\text{FE},L} N_{\text{QMC},L-l} 
    = \sum_{l=1}^{L} 2^{\gamma d l} 2^{2(L-l)} =  2^{2L} \sum_{l=1}^{L} 2^{ (\gamma d - 2) l}.
\]
These can further be reformulated as
\[
     W_{\text{MLMC},L} = 
    \begin{cases}
      L 2^{4L}  \text{  if  }  \gamma d = 4 , \\
      \dfrac{ 2^{\gamma d L} - 2^{4L}  }{2^{\gamma d - 4} - 1} \text{if  } \gamma d \neq  4 ,
    \end{cases}
\]
%
and
\[
     W_{\text{MLQMC},L} = 
    \begin{cases}
      L 2^{2L}  \text{  if  }  \gamma d = 2 , \\
      \dfrac{ 2^{\gamma d L} - 2^{2L}  }{2^{\gamma d - 2} - 1} \text{if  } \gamma d \neq  2 .
    \end{cases}
\]
Therefore, the asymptotical work behaviour for MLMC is bounded by 
$\mathcal{O}(2^{4L})$ when $\gamma d < 4$ (with an additional log-factor 
if $\gamma d = 4$), and by $ \mathcal{O}(2^{\gamma d L }) $ if $ \gamma d > 4$. 
Likewise, for MLQMC, the asymptotical work is bounded by $\mathcal{O}(2^{2L})$ 
when $\gamma d < 2$ (with an additional log-factor if $\gamma d = 2$), and 
by $ \mathcal{O}(2^{\gamma d L }) $ if $ \gamma d > 2$.

The complexity parameter $\gamma$ is therefore of major importance 
in the asymptotical work behaviour of the considered quadrature methods. 
In our case, given the Newton initial guess strategy, the solver preconditioning 
and the difference in parallel resources used from one level to another do not 
allow to give this parameter a concise value over all levels (compare Section 
\ref{sec:FEM}). We suggest however to evaluate the work in terms of total 
execution time, in which the cost $C_{\text{FE},l}$ for solving a sample at level 
$l$ is given by the time to solution (averaged over 100 samples). The 
resulting plot of work comparison between the different methods is 
reported in Figure \ref{fig::asymptotical-work-cube}.
On the on hand it is clearly visible that both MLMC and MLQMC show a significantly
improved asymptotic efficiency compared to their single level counterpart.
On the other hand comparing MLMC with MLQMC shows that MLQMC seems to be able to
use the higher convergence order of QMC versus MC to achieve
an improved asymptotic efficiency over MLMC.

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.6\textwidth]{figures/eps/Asymptotical_work_MC_MLMC_QMC_MLQMC_cube_singlethreaded.eps}
\captionsetup{justification=centering}
\caption{Work comparison for MC/MLMC/QMC/MLQMC. 
Work is computed on the basis of execution time on a single thread for all levels.}
\label{fig::asymptotical-work-cube}
\end{figure} 

%========================================
\subsubsection{Idealized ventricle}
%========================================
In the second test case, we rely on a mesh hierarchy of $L=3$ 
levels. The main reason for the limitation of levels number for this 
geometry is essentially due to the nestedness condition. Indeed, 
for this geometry as opposed to the simple cube one, we proceed 
in an inverted way, i.e.\ refining a given initial mesh. This procedure 
becomes demanding at the memory level very quickly since the 
refinement step increases the degrees of freedom by the factor 
$2^4 = 16$ due to the space--time discretization. In general, 
this limitation can very often be encountered when dealing with 
nested meshes for realistic geometries. This is the main motivation 
for relying on non-nested meshes for the last test case,
see Subsection \ref{subsection:anisotropic}.

The number of space-time degrees of freedom (DOF), the space 
and time discretization steps of the three different levels are 
reported in Table \ref{table:ventricle-levels}. The meshes 
are visualized in Figure \ref{fig::mesh-hierarchy-ventricle}.
The rates of convergence and the work of the different quadrature
methods are found in Figure \ref{fig::controlled-convergence-ventricle}.
As we have only three levels, the meaningfulness of the results is 
limited as it is impossible to conclude the asymptotic behaviour. 
Nevertheless, it is clearly seen that MLQMC is superior over the 
other methods.

\begin{table}[h!]
\centering
\begin{tabular}{|c||l|l|l|} 
\hline $l$ & 0 &  1 & 2   \\
\hline
% \hline $ N_x $  & 1'000 & 8'000 & 64'000    \\
% \hline $ N_t $  & 48 & 96 & 192    \\
\hline DOF  & 154'546 & 2'120'420 & 31'184'747   \\
\hline 
\hline 
$h$  & 0.1 & 0.05 & 0.025   \\
\hline
\hline
$\Delta t$  & 0.02 & 0.01 & 0.005   \\
\hline
\end{tabular}
\caption{Details about the mesh hierarchy for the idealized ventricle geometry.}
\label{table:ventricle-levels}
\end{table}

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.3\textwidth]{heart0.png}
\includegraphics[width=0.3\textwidth]{heart1.png}
\includegraphics[width=0.3\textwidth]{heart2.png}
\caption{Nested mesh hierarchy for the idealized ventricle.}
\label{fig::mesh-hierarchy-ventricle}
\end{figure} 

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/eps/QMC_MC_MLMC_MLQMC_Contolled_Convegence_ventricle_L2.eps}
\includegraphics[width=0.45\textwidth]{figures/eps/Asymptotical_work_MC_MLMC_QMC_MLQMC_ventricle.eps}
\captionsetup{justification=centering}
\caption{Convergence rate for the idealized ventricle in the $L^2$ norm (left)
and work comparison (right).}
\label{fig::controlled-convergence-ventricle}
\end{figure} 

%==========================================================
\subsection{Random fibers in a complex geometry with non-nested meshes} 
\label{subsection:anisotropic}
%==========================================================
The last test case concerns a realistic heart geometry with 
data acquired from clinical measurements. As this is meant to be 
the synthesis of this work, we also account for anisotropic 
diffusion defined in \eqref{eq:AdmV}. The associated expected 
fiber field $\mathbb{E}[{\bs V}] ({\bs x})$ is shown in Figure 
\ref{fig::initial-state-fibers}. It is obtained from a mathematical 
reconstruction using transmural coordinates~\cite{potse2006comparison}. 
The transmural coordinates are derived by initially solving a diffusion 
problem with adapted boundary conditions at the contour of the left 
and right ventricles~\cite{bayer2012novel}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.45\textwidth]{fibers_2.png}
\includegraphics[width=0.45\textwidth]{fibers_3.png}
\caption{Initial state for fibers $\mathbb{E}[{\bs V}] ({\bs x})$.}
\label{fig::initial-state-fibers}
\end{figure} 
%
We also relax the nestedness condition by considering a hierarchy of non-nested 
meshes. As we have previously argued, the nestedness condition 
very quickly becomes a burden in considering a large number of levels. 
We rely on a mesh hierarchy with 6 levels in this example. They are shown in Figure 
\ref{fig::mesh-hierarchy-heart}. The details on the space-time DOF 
and discretization steps are reported in Table \ref{table:heart-levels}.

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.3\textwidth]{lev0.png}
\includegraphics[width=0.3\textwidth]{lev1.png}
\includegraphics[width=0.3\textwidth]{lev2.png}
\includegraphics[width=0.3\textwidth]{lev3.png}
\includegraphics[width=0.3\textwidth]{lev4.png}
\includegraphics[width=0.3\textwidth]{lev5.png}
\caption{Non-nested mesh hierarchy for the realistic heart geometry.}
\label{fig::mesh-hierarchy-heart}
\end{figure} 

\begin{table}[h!]
\centering
\begin{tabular}{|c||l|l|l|l|l|l|} 
\hline $l$ & 0 &  1 & 2 & 3 & 4 & 5  \\
\hline
\hline DOF  & 18'480 & 113'312 & 583'104 & 1'740'800 & 8'777'728 & 34'894'848   \\
\hline
\hline $ h $  & 0.16 & 0.08 & 0.04 & 0.03 & 0.02 & 0.01   \\
\hline $ \Delta t $  & 0.16 & 0.08 & 0.04 & 0.02 & 0.01 & 0.005   \\
\hline 
\end{tabular}
\caption{Details about the mesh hierarchy for the realistic heart geometry.}
\label{table:heart-levels}
\end{table}

As we do not have nested finite element spaces, we rely here
on the multilevel estimator \eqref{eq:PimpedML}. Moreover, 
we evaluate the convergence for the two quantities of interest, 
namely the action potential and the activation times for given 
locations in the domain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%               Action potential      %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Action potential}
We evaluate the evolution of the action potential in several 
locations of the heart domain. The first example considers a 
set of points that are placed along the wall separating the left 
and right ventricles. These points are shown in Figure \ref{fig::wall-points}. 

\begin{figure}[h!]
\centering
\begin{tikzpicture}
\draw(0,0)node{\includegraphics[width=0.49\textwidth]{horizontal_longitudinal.png}};
% \includegraphics[width=0.49\textwidth]{horizontal_longitudinal_blackexternalpointlabels.png}
\draw[line width=0.8pt] (-0.12,-1.53)--(3.6,-1.53);
\draw[line width=0.8pt] (-0.52,-0.66)--(3.6,-0.66);
\draw[line width=0.8pt] (-0.64,0.16)--(3.6,0.16);
\draw[line width=0.8pt] (-0.55,0.86)--(3.6,0.86);
\draw[line width=0.8pt] (-0.27,1.46)--(3.6,1.46);
\draw[line width=0.8pt] (0.14,2.12)--(3.6,2.12);
\draw (3.8,-1.53)node{P1};
\draw (3.8,-0.66)node{P2};
\draw (3.8,0.16)node{P3};
\draw (3.8,0.86)node{P4};
\draw (3.8,1.46)node{P5};
\draw (3.8,2.12)node{P6};
\end{tikzpicture}

\caption{Locations selected along the wall separating the left and right ventricles.}
\label{fig::wall-points}
\end{figure} 

As one can see, these points have been selected such that they 
trace the behaviour of locations at different distance from the stimulus 
center, starting from very close (the very below point) to relatively 
far (the very top point). We report in Figure~\ref{fig::AP-wall} the 
action potential obtained by the MC quadrature method for different 
discretization levels.
%The order goes from the top left for the very bottom 
%point defined in Figure \ref{fig::wall-points} to the below right for the 
%upper point. 

\begin{figure}[H] %[h!]
\begin{tikzpicture}
\draw(0,0)node{
\includegraphics[width=0.3\textwidth]{MC-5-levels-idx=6.png}};
\draw(5,0)node{
\includegraphics[width=0.3\textwidth]{MC-5-levels-idx=5.png}};
\draw(10,0)node{
\includegraphics[width=0.3\textwidth]{MC-5-levels-idx=4.png}};
\draw(0,-3.5)node{
\includegraphics[width=0.3\textwidth]{MC-5-levels-idx=3.png}};
\draw(5,-3.5)node{
\includegraphics[width=0.3\textwidth]{MC-5-levels-idx=2.png}};
\draw(10,-3.5)node{
\includegraphics[width=0.3\textwidth]{MC-5-levels-idx=1.png}};
\draw(0,1.5)node{P1};
\draw(5,1.5)node{P2};
\draw(10,1.5)node{P3};
\draw(0,-2)node{P4};
\draw(5,-2)node{P5};
\draw(10,-2)node{P6};
\end{tikzpicture}
% \includegraphics[width=0.3\textwidth]{MC-5-levels-idx=6_P1.png}
% \includegraphics[width=0.3\textwidth]{MC-5-levels-idx=5_P2.png}
% \includegraphics[width=0.3\textwidth]{MC-5-levels-idx=4_P3.png}
% \includegraphics[width=0.3\textwidth]{MC-5-levels-idx=3_P4.png}
% \includegraphics[width=0.3\textwidth]{MC-5-levels-idx=2_P5.png}
% \includegraphics[width=0.3\textwidth]{MC-5-levels-idx=1_P6.png}
\captionsetup{justification=centering}
\caption{Action potential behaviour given different mesh level discretizations 
for the points specified in Figure \ref{fig::wall-points} following the order going from the bottom to the top.}
\label{fig::AP-wall}
\end{figure} 

In Figure \ref{fig::AP-convergence-1}, we report the convergence graphs 
of the (pointwise) error \eqref{eq:point-error} for the action potential 
at the locations introduced in Figure \ref{fig::wall-points} and $q=1$.
Notice that the graphs report the root mean square errors.
The expected convergence rate is achieved for all quadrature methods tested.

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.3\textwidth]{figures/eps/AP_wall_pt_1.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_wall_pt_2.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_wall_pt_3.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_wall_pt_4.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_wall_pt_5.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_wall_pt_6.eps}
\captionsetup{justification=centering}
\caption{Convergence in the $H^1$ norm of the action potential at the 
locations specified in Figure \ref{fig::wall-points} following the order going from the bottom to the top.}
\label{fig::AP-convergence-1}
\end{figure} 

The second test is concerned with points located at the circumference 
of a horizontal cut of the heart surface. These are shown in Figure 
\ref{fig::circonference-points}.
\begin{figure}[h!]
\centering
\includegraphics[width=0.49\textwidth]{horizontal_circonference_2.png}
\captionsetup{justification=centering}
\caption{Locations selected at the circumference of a horizontal cut of the heart surface.}
\label{fig::circonference-points}
\end{figure} 

Since the behaviour of the action potential at these points follows
a similar pattern to that of the previously shown ones, cf.\ Figure 
\ref{fig::AP-wall}, we directly show the graph regarding the convergence of 
the action potential at these points in Figure \ref{fig::AP-convergence-2}.
Again, we see the expected convergence rate for all quadrature methods tested.

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_1.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_2.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_3.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_4.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_5.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_6.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/AP_circonference_pt_7.eps}
\captionsetup{justification=centering}
\caption{Convergence of the action potential at the locations 
specified in Figure \ref{fig::circonference-points}
following the order going from left to right.}
\label{fig::AP-convergence-2}
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%               Activation time      %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%=========================================
\subsubsection{Activation time}
%=========================================
We start by selecting points at equivalent geodesic 
distance from the stimulus location. These points are 
shown in Figure \ref{fig::activation-contour}. The geodesic 
distance is calculated by solving an eikonal problem with a 
zero initial condition on the originating point~\cite{pezzuto2019sampling}, 
i.e.\ the stimulus in our case. The graphs showing the 
convergence of the activation times for these locations
are reported in Figure \ref{fig::activation-graph-1},
with all of them showing the expected rate of convergence for all quadrature methods tested.

\begin{figure}[h!] % [H] 
\centering
\includegraphics[width=0.45\textwidth]{pts_on_contour.png}
\includegraphics[width=0.45\textwidth]{pts_on_contour_2.png}
\caption{Locations selected at equivalent geodesic distance from the stimulus.}
\label{fig::activation-contour}
\end{figure} 

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.3\textwidth]{figures/eps/activation_contour_pt_1.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_contour_pt_2.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_contour_pt_3.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_contour_pt_4.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_contour_pt_5.eps}
\captionsetup{justification=centering}
\caption{Convergence of the activation time at the 
locations specified in Figure \ref{fig::activation-contour} following the order going from left to right.}
\label{fig::activation-graph-1}
\end{figure} 

We next select locations at the circumference of the left ventricle. 
These are shown in Figure \ref{fig::activation-transversal}. 
%These 
%can be interpreted as clinically disposed electrodes %on some locations 
%of the torso.
This electrical signal, when propagated to the chest,
is exactly what is perceived clinically (on a 
electrocardiogram monitor).
Mathematically, it is possible to map the surface
potential to the chest by solving an additional
diffusion problem, see \cite{fernandez2010decoupled,
boulakia2010mathematical}.
As we have several 
discretization levels, we need to ensure that these points are 
well-defined on each one of them. The convergence graphs for the activation
times at these locations,
which validate the the expected rate of convergence
for all quadrature methods tested,
are reported in Figure \ref{fig::activation-graph-2}.

\begin{figure}[htb] %[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/clean/activation_transversal_2.png}
\includegraphics[width=0.45\textwidth]{figures/clean/activation_transversal.png}
\captionsetup{justification=centering}
\caption{Locations selected at the periphery of the heart surface.}
\label{fig::activation-transversal} 
\end{figure} 

\begin{figure}[H] %[h!]
\centering
\includegraphics[width=0.3\textwidth]{figures/eps/activation_transversal_pt_1.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_transversal_pt_2.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_transversal_pt_3.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_transversal_pt_4.eps}
\includegraphics[width=0.3\textwidth]{figures/eps/activation_transversal_pt_5.eps}
\captionsetup{justification=centering}
\caption{Convergence of the activation time at the 
locations specified in Figure \ref{fig::activation-transversal} following an order going from the furthest of the (final state) travelling wave to the nearest.}
\label{fig::activation-graph-2}
\end{figure} 

% The non-nestedness of the finite element spaces  

